Large-Scale Contextual Market Equilibrium Computation through Deep Learning

Market equilibrium is one of the most fundamental solution concepts in economics and social optimization analysis. Existing works on market equilibrium computation primarily focus on settings with relatively few buyers. Motivated by this, our paper investigates the computation of market equilibrium in scenarios with a large-scale buyer population, where buyers and goods are represented by their contexts. Building on this realistic and generalized contextual market model, we introduce MarketFCNet, a deep learning-based method for approximating market equilibrium. We start by parameterizing the allocation of each good to each buyer using a neural network, which depends solely on the context of the buyer and the good. Next, we propose an efficient method to unbiasedly estimate the loss function of the training algorithm, enabling us to optimize the network parameters through gradient. To evaluate the approximated solution, we propose a metric called Nash Gap, which quantifies the deviation of the given allocation and price pair from the market equilibrium. Experimental results indicate that MarketFCNet delivers competitive performance and significantly lower running times compared to existing methods as the market scale expands, demonstrating the potential of deep learning-based methods to accelerate the approximation of large-scale contextual market equilibrium.

==> Contents/Body/5_Trans.tex <==
\section{MarketTransNet}
\label{sec:TransNet}


In this section, we introduce the MarketTransNet (denoted as Market Transform-based Network) to approximate market equilibria on a large number of markets using the idea of function approximation. 
Function approximation implies that by inputting a market in its raw form, one can directly obtain the results of allocations and prices without necessitating any intermediate processing. 
Given a representation of a market, MarketTransNet can output an approximate market equilibrium by taking the representation as input.
To the best of our knowledge, this is the first work that attempts to compute the market equilibrium by function approximation. 
The key is to redefine the problem so that the network can simultaneously compute the allocation results and the final prices of goods, ensuring that these two outcomes satisfy the market clearance and price constraints.


\subsection{Problem Reformulation}
Consider $K$ markets, denoted as $\calM^1,...,\calM^K$, where $K$ can potentially be infinitely large.
In the $k$'th market $\calM^k$, we have $n$ buyers and $m$ goods waiting to be allocated.  $b^k_i \in \calB$ and $g^k_j \in \calG$ are denoted as the $i$'th buyer and the $j$'th good. Similarly, the superscript $k$ indicates that it comes from the $k$'th market. However, the budget function and value function remain the same on different markets.

Given buyer representation $\bmb^k \in \calB^n$ and good representation $\bmg^k \in \calG^m$, our output should be allocation results $\bmx^k \in \bbR^{n \times m}_+$ together with prices for goods $\bmp^k \in \bbR^{m}_+$. 
The network is a mapping $f_\theta : [\bmb,\bmg] \rightarrow [\bmx, \bmp]$.
As discussed in \cref{sec:preliminary} and \cref{sec:performance}, the market equilibrium satisfies market clearance and price constraints. Hence, we aim for the network's output to automatically satisfy the following conditions:
\begin{align}
    \quad \sum_\iinn x_{ij} = n, 
    \quad x_{ij}\ge 0,\quad \forall i\in[n],\ j \in [m] \\
    \quad \sum_j p_j = \frac{1}{n}\sum_\iinn B(b_i)
    \quad p_j\ge 0,\quad \forall j \in [m]
\end{align}

Our network $f_\theta$ should also possess the following three characteristics: 
\begin{itemize}
    \item The network should process input with variable-length inputs, and the model needs to respond to markets with different numbers of buyers and goods. 

    \item $f_\theta$ should have Permutation-Equivariance. The output allocation and price should be equivariant to any permutation of the row index and column index, since no permutation of buyers and goods should affect the market equilibrium as a whole.

    \item Satisfying constraints. Our network must use an explicit method to satisfy market clearance and price constraints.
\end{itemize}


Much work has been done to identify neural network structures that exhibit the special properties mentioned above. Our specific implementation follows the work of \cite{duan2022context} and adopts a transformer architecture for handling multi-market data. 

Here all constraints are automatically satisfied by the transformer architecture.
The Transformer is \textbf{independent of the length of the sequence}. 
% Specifically, operations such as feed-forward and add \& norm are point-wise and will do their jobs recurrently. The attention layer computes the score matrix and outputs the weighted and adjusted new sequence, which is also independent of the sequence length. (byd wondering if it is necessary to explain the comment line)
This characteristic gives more flexibility to model and allows us to train the network on markets of smaller scales, and generalize it to markets with larger size. 
The self-attention mechanism in transformers inherently provides \textbf{permutation-equivariance}. If the order of the input sequence changes, the weighting order of the self-attention is adjusted accordingly to keep the output consistent.
Moreover, let $F^x \in \calR^{n\times m}$, $F^p \in \calR^{m}$ denote the final feature maps prior to outputting the ultimate allocation results and prices, it undergoes the subsequent processing:
\begin{align}
    \bmx_{\cdot,j} &= \text{Softmax}(F^x_{\cdot,j}) \times n, \quad \forall j \in [m]. \qquad 
    \bmp_{\cdot} = \text{Softmax}(F^p_{\cdot}) \times \frac{1}{n}\sum_{i=1}^n B(b_i).
\end{align}
% First Step ensures that the number of good j acquired by each individual sums up to the initial endowment of  good j. The following  one makes the value of all items equals the sum of all buyers' budgets. 
By the nature of the softmax function, we have allocation $\sum_{i=1}^n x_{ij} = n$,$x_{ij} \ge 0$ and price $\sum_j p_j = \frac{1}{n}\sum_{i=1}^n B(b_i)$, all of which \textbf{meet the constraints}.

Our MarketTransNet consists of three components:(1) Cross-broadcasting representation about buyers and goods to form a correlated buyer-good pair. (2) Taking row interactions/column interactions/global averaging on each pair and gluing them together. (3) Reduce the feature dimension to $2$ and do the softmax processing mentioned above. Readers can move to \cref{app:trans-architecture} for more details.

According to Theorem 3.5, to directly solve the market equilibrium for each market, we need to minimize the \emph{Nash Gap} for each market. In MarketTransNet, we consider minimizing the average \emph{Nash Gap} for all markets throughout the optimization.
\begin{equation}
\label{eq:optim:trans1}
\begin{aligned}
    \min _\theta &\quad \frac{1}{K}\sum_{k=1}^K \GAP(\bmb^k,\bmg^k;\theta)\\
    % = &\phantom{-} \frac{1}{K} \sum_{k=1}^K \sum_{i=1}^n B\left(b^k_i\right) 
    %  \Bigl[ \log u \left(b^k_i, \bmp \left( \bmb^k, \bmg^k ; \theta \right) \right)  \\
    % & \phantom{\frac{1}{K} \sum_{k=1}^K \sum_{i=1}^n B(b^k_i) \Bigl[} - \log u \left(b^k_i,\bmx_i \left( \bmb^k, \bmg^k ; \theta \right)\right) \Bigr] \\
    s.t.&\quad \sum_\iinn x_{ij} = n, 
    \quad x_{ij}\ge 0,\quad \forall i\in[n],\ j \in [m] \\
    &\quad \sum_j p_j = \frac{1}{n}\sum_\iinn B(b^k_i)
    \quad p_j\ge 0,\quad \forall j \in [m]
\end{aligned}
\end{equation}

Here we denote $\GAP(\bmb,\bmg;\theta)$ to be the \emph{Nash Gap} when buyers and goods are $\bmb$ and $\bmg$ and the model is parameterized with $\theta$.
Given the large size of $K$, computing the average \emph{Nash Gap} is intractable. Therefore, we consider to randomly choose $M$ batch of markets to train the network on each iteration. 

% \begin{algorithm}[t]
% \caption{MarketTransNet}
% \begin{algorithmic}
% \STATE \textbf{Input:} A market sampler, number of buyers $n$, number of goods $m$, batch size $M$.
% \STATE \textbf{Output:}Transformer network $\calX(\bmb,\bmg;\theta)$ including allocation $\bmx(\bmb,\bmg;\theta)$ and price $\bmp(\bmb,\bmg;\theta)$
% \STATE Initialize a transformer network $\calX(\bmb,\bmg;\theta)$.
% \FOR{$t = 1,2,...$ until converged}
%     \STATE Generate $M$ batch of random market instance with $n$ buyers and $m$ goods.
%     \STATE Compute the loss function $\mathrm{average \emph{Nash Gap}}(\theta)$ on these instances.
%     \STATE Compute the gradient $Gradient$
%     \STATE $\qquad\qquad\qquad\quad\qquad= \nabla_\theta \mathrm{average \emph{Nash Gap}}(\theta)$.
%     \STATE Update $\theta$ with $Optimizer(\theta, Gradient)$.
% \ENDFOR
% \STATE \textbf{return:}$\calX(\bmb,\bmg;\theta)$: Transformer network that can determine allocation and price for one market.
% \end{algorithmic}
% \end{algorithm}


